Quantum decorated character stacks

We initiate the study of decorated character stacks and their quantizations using the framework of stratified factorization homology. We thereby extend the construction by Fock and Goncharov of (quantum) decorated character varieties to encompass also the stacky points, in a way that is both compatible with cutting and gluing and equivariant with respect to canonical actions of the modular group of the surface. In the cases $G=SL_2,PGL_2$ we construct a system of categorical charts and flips on the quantum decorated character stacks which generalize the well--known cluster structures on the Fock--Goncharov moduli spaces.

==> jellyfish.tex <==
\begin{tikzpicture}[every node/.style={inner sep=0, minimum size=0.1cm, thick, circle}, thick, x=0.35cm, y=0.35cm]


\end{tikzpicture}
